Tree-Structured Clustering in Fixed Effects Models

Fixed effects models are very flexible because they do not make assumptions on the distribution of effects and can also be used if the heterogeneity component is correlated with explanatory variables. A disadvantage is the large number of effects that have to be estimated. A recursive partitioning (or tree based) method is proposed that identifies clusters of units that share the same effect. The approach reduces the number of parameters to be estimated and is useful in particular if one is interested in identifying clusters with the same effect on a response variable. It is shown that the method performs well and outperforms competitors like the finite mixture model in particular if the heterogeneity component is correlated with explanatory variables. In two applications the usefulness of the approach to identify clusters that share the same effect is illustrated.

==> header.tex <==
%% neu 1.9.2011     Abstände zwischen den Einträgen des Literaturverzeichnisses variieren.



%% Schrift
%\usepackage{mathptmx}
%\usepackage[scaled=.90]{helvet}
%\usepackage{courier}



\usepackage{times}      % old but good
%\usepackage{lmodern} %Latex STandard Schrift


%% language, coding
\usepackage[german,english]{babel}
\usepackage[T1]{fontenc}
\usepackage{textcomp}
\usepackage[latin1]{inputenc}

\usepackage{afterpage}

\usepackage{multind}             %multiple Inidices



\usepackage{chicago_new}




\usepackage{amsfonts, amsmath, amssymb, amsthm}
\usepackage{calc}
\usepackage{curves,epic,eepic,latexsym,ifthen}
%new
\usepackage{curves,epic,eepic,amsmath,latexsym,amssymb,array,ifthen,dcolumn}
\usepackage{epsfig}

%new
\usepackage{graphicx}
\usepackage[only,tenrm,svtnrm,egtrm,frtnrm]{rawfonts}

%\usepackage{showkeys}   %Label-Name at margin

\usepackage{rotating}
\usepackage{bbm}

\usepackage{color}
\usepackage{verbatim}
\usepackage{float}
\usepackage{textcomp}
\usepackage[english]{varioref}
\usepackage[scanall]{psfrag}

%Schauberger
\usepackage{tikz}
\usepackage{tikz-qtree}
\usepackage{pgfkeys}

\listfiles

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Tables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{%
  longtable,
  array,
  booktabs,
  dcolumn,
  rotating,
  shortvrb,
  tabularx,
  units,
  multirow
}

%\usepackage{fltpoint}
%\usepackage{rccol}
%\rcDecimalSign{.}


%% booktabs
\setlength{\heavyrulewidth}{0.06em}    % for \toprule and \bottomrule (default 0.08em)
\setlength{\lightrulewidth}{0.04em}    % for \midrulelightrulewidth (default 0.05em)
    % cmidrulewidht = 0.03em (fr \cmidrule)


%% Tables specific letter type
\newenvironment{tabularsmall}
{
\footnotesize \sffamily
\tabular
}
{
\endtabular
\normalfont
}

%% Ausrichtung am Dezimalpunkt
\newcolumntype{d}[1]{D{.}{.}{#1}} %% d{Anz.Dezimalstellen}


\newcolumntype{.}[1]{D{.}{.}{#1}}  %% in count


%% zum leichteren Ausrichten von Tabellenspalten
\newcommand{\ph}[1]{\phantom{#1}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Pages, Margins
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[
DIVcalc,       % Textbereich (in log-Datei nachlesen)
%DIVclassic
%,headinclude    % dann ist Kopfzeile+Text 18,9cm hoch,
%,headexclude    % dann ist nur der Text 18.9cm hoch + Kopfzeile
%,footexclude    % footinclude
,1.0headlines   %default ist 1.25headlines
%,pagesize
]{typearea}

%\typearea{8}

%\areaset{11.7cm}{18.9cm}
\areaset{13.3cm}{21.0cm}
%kleinerer Abstand von Kopfzeile zu Text
%\setlength{\headheight}{0pt} %13.6pt    holt den Text etwas nï¿½er



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         fancy head and bottom
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{fancyhdr}

\pagestyle{fancy}
\lhead[\fancyplain{}{\textrm\thepage}]                            % even page
      {\fancyplain{}{\normalfont\footnotesize\scshape\rightmark}} % uneven page
\rhead[\fancyplain{}{\normalfont\footnotesize\scshape\leftmark}]
      {\fancyplain{}{\textrm\thepage}}
\chead{}

\renewcommand{\headrulewidth}{0.5pt} % Trennlinie
\setlength{\headsep}{10pt}           % kleinerer Abstand Text-Kopfzeile (default ist 25pt)

\lfoot{}
\cfoot{\fancyplain{\textrm\thepage}{}}
\rfoot{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  minipages with boxes
% use  \boxnew[Breite]{Inhalt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\boxtitle}[1]{\begin{center} \sffamily #1 \end{center}}
\newcommand{\boxitem}[1]{\textsf{\small #1}}

\newcommand{\boxnew}[2][0.8\textwidth]{               %0.8\textwidth als default
   \vspace{1.5ex}          %1ex bewirkt nichts, entspricht 100%
   \begin{center}
   \fbox{%
     \begin{minipage}{#1}   %\linewidth-4ex  ergibt textbreiten Kasten
       {#2}%
     \end{minipage}}%
   \end{center}
   \vspace{2ex}
}

\newcommand{\boxcaption}[1]{
\captionsetup{aboveskip=-1.6ex, belowskip=2ex}
\captionof{table}{#1}
\captionsetup{aboveskip=10pt, belowskip=0pt}
\vspace{1.5ex}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Index (neu 6.7.06 von J.Brandt)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\sindex}[1]{\index{subjectindex}{#1}}
\newcommand{\aindex}[1]{\index{authorindex}{#1}}

% Zweispaltiger Index
\makeatletter
\renewcommand{\printindex}[2]{
   \@restonecoltrue\if@twocolumn\@restonecolfalse\fi
   \columnseprule \z@ \columnsep 35pt   %%obsolet, besser \setlength
   \newpage
   \@mkboth{\MakeUppercase{#2}}{\MakeUppercase{#2}}      %Fr Kopfzeile
%    \twocolumn[{\rm\huge\sffamily\mdseries #2 \vskip4ex}]      %%obsolet, wegen \rm
    \twocolumn[{\rm\huge\sffamily\mdseries #2 \vskip4ex}]
   \addcontentsline{toc}{chapter}{#2}                    %Eintrag ins Inhaltsverzeichnis
   \@input{#1.ind}
 }
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Examples including counter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\newcommand{\ecaption}[1]{\addcontentsline{loe}{example}{\protect\numberline{\theexample}#1}} %loe: listOfExamples
\newcommand{\l@example}{\@dottedtocline{1}{0em}{3.2em}}

\newcommand{\listofexamples}{
     \chapter*{List of Examples}                  %ï¿½berschrift der Beispielsliste
     \@mkboth{List of Examples}{List of Examples}         %header
%   \addcontentsline{toc}{section}{List of Examples}    %hier liegt das Problem mit den minitocs => statt chapter nun section und es funktioniert
\addcontentsline{toc}{chapter}{List of Examples}
%     \thispagestyle{empty}
     { \@starttoc{loe}}
}
\makeatother

\newcounter{example}[chapter]
\renewcommand{\theexample}{\thechapter.\arabic{example}}

\newenvironment{example}[1]
    {\refstepcounter{example}
     \ecaption{#1}
     \bigskip
     \noindent{\small \sffamily Example \theexample: #1}
     %\noindent{\small \scshape Example \normalfont \theexample: #1}
                    % Schrift der Beispielsberschrift
     \small         % Schrift des Textes (ohne ï¿½berschrift)
     \\}
    {\qed \bigskip}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Chapter headings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
%% aus book.cls kopiert und modifiziert
\renewcommand\chapter{\if@openright\cleardoublepage\else\clearpage\fi
                    \thispagestyle{plain}%
                    \global\@topnum\z@
                    \@afterindentfalse
                    \secdef\@chapter\@schapter}
\def\@chapter[#1]#2{\ifnum \c@secnumdepth >\m@ne
                       \if@mainmatter
                         \refstepcounter{chapter}%
                         \typeout{\@chapapp\space\thechapter.}%
                         \addcontentsline{toc}{chapter}%
                                   {\protect\numberline{\thechapter}#1}%
                       \else
                         \addcontentsline{toc}{chapter}{#1}%
                       \fi
                    \else
                      \addcontentsline{toc}{chapter}{#1}%
                    \fi
                    \chaptermark{#1}%
                    \addtocontents{lof}{\protect\addvspace{10\p@}}%
                    \addtocontents{lot}{\protect\addvspace{10\p@}}%
                    \if@twocolumn
                      \@topnewpage[\@makechapterhead{#2}]%
                    \else
                      \@makechapterhead{#2}%
                      \@afterheading
                    \fi}
\def\@makechapterhead#1{%
  \vspace*{50\p@}%
  {\parindent \z@ \raggedright \sffamily  %\normalfont default, jetzt \sffamily
    \ifnum \c@secnumdepth >\m@ne
      \if@mainmatter
        \huge \@chapapp\space \thechapter %\bfseries  %nur fï¿½r das Wort Chapter
        \par\nobreak
        \vskip 20\p@        %20
      \fi
    \fi
    \interlinepenalty\@M
%    \Huge  #1\par\nobreak  %\bfseries       %fï¿½r die eigentliche ï¿½berschrift
    \huge  #1\par\nobreak  %\bfseries
    \vskip 40\p@        %40
  }}
\def\@schapter#1{\if@twocolumn
                   \@topnewpage[\@makeschapterhead{#1}]%
                 \else
                   \@makeschapterhead{#1}%
                   \@afterheading
                 \fi}
\def\@makeschapterhead#1{           %verï¿½ndert die Schrift der ï¿½berschrift des Inhalts-, Beispiels- und Literaturverzeichnisses
  \vspace*{50\p@}%
  {\parindent \z@ \raggedright
    \sffamily                       %\normalfont alt
    \interlinepenalty\@M
%    \Huge   #1\par\nobreak          %\bfseries
    \huge   #1\par\nobreak
    \vskip 40\p@
  }}
%%

\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {-3.5ex \@plus -1ex \@minus -.2ex}% Abstand drï¿½ber
                                   {1.1ex \@plus.1ex}      % Abstand drunter
                                   {\sffamily\Large}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                     {-3.25ex\@plus -1ex \@minus -.2ex}%
                                     {1.0ex \@plus .1ex}%
                                     {\sffamily\large}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                     {-3.25ex\@plus -1ex \@minus -.2ex}%
                                     {0.5ex \@plus .1ex}%
                                     {\sffamily\normalsize}}
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
                                    {3.25ex \@plus1ex \@minus.2ex}%
                                    {1ex}%
                                    {\sffamily\normalsize}}
\makeatother

%default-Werte
% \newcommand\section{\@startsection {section}{1}{\z@}%
%                                    {-3.5ex \@plus -1ex \@minus -.2ex}%
%                                    {2.3ex \@plus.2ex}%
%                                    {\normalfont\Large\bfseries}}
% \newcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                      {-3.25ex\@plus -1ex \@minus -.2ex}%
%                                      {1.5ex \@plus .2ex}%
%                                      {\normalfont\large\bfseries}}
% \newcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%                                      {-3.25ex\@plus -1ex \@minus -.2ex}%
%                                      {1.5ex \@plus .2ex}%
%                                      {\normalfont\normalsize\bfseries}}
% \newcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
%                                     {3.25ex \@plus1ex \@minus.2ex}%
%                                     {-1em}%
%                                     {\normalfont\normalsize\bfseries}}
% \newcommand\subparagraph{\@startsection{subparagraph}{5}{\parindent}%
%                                        {3.25ex \@plus1ex \@minus .2ex}%
%                                        {-1em}%
%                                       {\normalfont\normalsize\bfseries}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Im Anhang bekommen chapter, section und subsection wieder andere Bedeutung
% (noch nicht berarbeitet)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \makeatletter
%   \renewcommand*\l@chapter[2]{%
%     \ifnum \c@tocdepth >\m@ne
%       \addpenalty{-\@highpenalty}%
%       \vskip 1.0em \@plus\p@
%       \setlength\@tempdima{1.5em}%
%       \begingroup
%         \parindent \z@ \rightskip \@pnumwidth
%         \parfillskip -\@pnumwidth
%         \leavevmode \bfseries %\mdseries %\sffamily
%         \advance\leftskip\@tempdima
%         \hskip -\leftskip
%         #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\par
%         \penalty\@highpenalty
%       \endgroup
%     \fi}
% \renewcommand{\appendixname}{Appendix}
% \renewcommand{\appendix}{%
%   \setcounter{chapter}{0}
%   \renewcommand{\thechapter}{\Alph{chapter}}%
%   \renewcommand{\chapter}[1]{%
%     \cleardoublepage\thispagestyle{plain}%
%     \refstepcounter{chapter}%
%     \addcontentsline{toc}{chapter}%
%       {%\protect\sffamily%
%        \protect\numberline{\protect\bfseries\protect%   %%dazw.\bfseries
%        \protect\appendixname\protect\hspace{1ex}\thechapter:}\protect\hspace{9ex}\protect##1}%
%     \@mkboth{\MakeUppercase{\appendixname\ \thechapter:\ ##1}}%
%             {\MakeUppercase{\appendixname\ \thechapter:\ ##1}}%
%     {\flushleft\LARGE\mdseries\sffamily%
%      \appendixname\ \thechapter:\ \nohyphens##1\par}%
%   %\chaptermark{##1}\vspace{\baselineskip}
%   }
%   \renewcommand{\section}[1]{
%     \refstepcounter{section}%
%     \addcontentsline{toc}{section}%
%       {%\protect\sffamily%
%        \protect\numberline{\thesection}##1}%
%     {\noindent\large\mdseries\sffamily\thesection~##1\par}
% %    {\flushleft\large\mdseries\sffamily\thesection~##1\par} ohne Trennungen
%   }
%   \renewcommand{\subsection}[1]{
%     \refstepcounter{subsection}%
%     \addcontentsline{toc}{subsection}%
%       {%\protect\sffamily%
%        \protect\numberline{\thesubsection}##1}%
%     {\noindent\normalsize\mdseries\sffamily\thesubsection~##1\par}
% %    {\flushleft\normalsize\mdseries\sffamily\thesubsection~##1\par} ohne Trennungen
%   }
% }
%% \makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Captions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{caption}[2003/12/20]
\captionsetup{width=\linewidth-2cm,font=footnotesize,labelfont={sc}}
    %font: Einstellung fï¿½r die gesamte Unterschrift
    %labelfont: Einstellung fï¿½r den Bezeichner (``Table'')


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Literature  - neu 1.9.2011 JB
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% aus book.cls %%

\makeatletter

\renewenvironment{thebibliography}[1]
     {\chapter*{\bibname}%
      \@mkboth{\MakeUppercase\bibname}{\MakeUppercase\bibname}%
      %     {\rm\Large\sffamily\mdseries \bibname\vskip2ex}     %ergänzt
    \addcontentsline{toc}{chapter}{\bibname}    %ergänzt
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist}

\makeatother

\let\oldbibliography\thebibliography
\renewcommand{\thebibliography}[1]{%
\oldbibliography{#1}%
%\setlength{\itemsep}{0ex}           %% Abstand zwischen den Einträgen %%
\setlength{\itemsep}{-0.3ex} }




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         minitocs: kleine Inhaltsverzeichnisse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{minitoc}       % kleine Inhaltsverzeichnisse
\setlength{\fboxsep}{1em}  % \fboxsep4mm    %Vergleiche Einstellungen fï¿½r \boxnew
\setlength{\mtcindent}{4pt}
\renewcommand{\mtcfont}{\small\mdseries\sffamily}
\renewcommand{\mtcSfont}{\small\mdseries\sffamily}
\renewcommand{\mtcSSfont}{\small\mdseries\sffamily}

\newcommand{\makeminitoc}{%
\setcounter{minitocdepth}{3}    % Anzahl Gliederungsebenen
   \vspace{3mm}
   \hrule
   \bigskip
   \noindent


%   \fbox{%
   \begin{minipage}{\linewidth -5ex}
     \vspace*{-3ex}
     \nomtcrule
     \minitoc
\hrule
\bigskip
%     \vspace*{-5ex}%3
   \end{minipage}
%   }
\\[3mm]}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%          Applications   ** neu 21.10.09 JB
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ZÃ¤hler fÃ¼r die Applications innerhalb der Umgebung
\newcounter{application}[chapter]
\renewcommand{\theapplication}{\thechapter.\arabic{application}}

%% Definition der Umgebung 'application'
\newenvironment{application}
    {\refstepcounter{application}
     \bigskip
     \noindent{\small \sffamily Application \theapplication:} % Ãberschrift
     \\
     \small         % Schrift des Textes (ohne Ueberschrift)
     }

    { \bigskip}

%% Fuer leichtere (a), (b), (c) AufzÃ¤hlungen
\usepackage{enumitem}

\newenvironment{abcitemize}
    {\begin{enumerate}[label=(\alph*)]}
    {\end{enumerate}}


% \newenvironment{anwendung}[1]
%     {\refstepcounter{application}
%      \bigskip
%      \noindent{\small \sffamily Application \theapplication:} % Ãberschrift
%      \small         % Schrift des Textes (ohne Ueberschrift)
%      \\
%      #1
%      \begin{enumerate}[label=(\alph*)]
%      }
%     { \end{enumerate} \bigskip}







% %% Variante 2 *****************************************************************

%
%
% \renewcommand{\labelenumi}{\small \textsf{Application \theenumi :}}
%
%
% \newenvironment{anwendungen}%[Ã]
% {\small \begin{enumerate}[leftmargin=*, style=nextline] }
% {\end{enumerate} }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%          Exercises   ** neu 19.11.09 JB
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ZÃ¤hler fÃ¼r die Exercieses
\newcounter{exercise}[chapter]
\renewcommand{\theexercise}{\thechapter.\arabic{exercise}}

%% Definition der Umgebung 'exercise'
\newenvironment{exercise}
    {\refstepcounter{exercise}
     \bigskip \small
     \noindent \theexercise
     }

    { \bigskip}

